Distributed Set-Based Observers Using Diffusion Strategies

We propose two distributed set-based observers using strip-based and set-propagation approaches for linear discrete-time dynamical systems with bounded modeling and measurement uncertainties. Both algorithms utilize a set-based diffusion step, which decreases the estimation errors and the size of estimated sets, and can be seen as a lightweight approach to achieve partial consensus between the distributed estimated sets. Every node shares its measurement with its neighbor in the measurement update step. In the diffusion step, the neighbors intersect their estimated sets using our novel lightweight zonotope intersection technique. A localization example demonstrates the applicability of our algorithms.

==> Sections/2-intro_short.tex <==
\section{Introduction}


%State estimation across wireless networks is often a key technology for emergency rescue missions, homeland security \citep{conf:homeland}, habitat monitoring \citep{conf:habitat}, and home automation services \citep{conf:homeauto}. 

%State estimation algorithms are categorized according to the type of modeled uncertainties, which are either stochastic or set-based approaches. 
State estimation algorithms either compute a single state, a probability distribution of the state, or bound the set of possible states by sets. In stochastic approaches, measurement and process noises are modeled by provided statistical distributions (e.g., Gaussian \citep{conf:kfintro}). On the other hand, set-based approaches assume noises to be unknown but bounded by known bounds. Safety-critical applications require guarantees on the state estimation during operation -- such guarantees can be provided by the set-based approaches. %Also, set-based approaches are traditionally used in fault detection by generating an adaptive threshold to check the consistency of the measurements with the estimated output set \citep{conf:intervalVSset-membership,conf:set_fault1,conf:faultcombastel1,conf:set_fault3,conf:actuator_fault,conf:fdi}. Among the family of set-based approaches, interval-based and set-membership observers have been introduced separately \citep{conf:intervalVSset-membership}. We focus in the subsequent literature survey on both approaches. 


%They are very useful for fault detection \citep{}

%While some observers neglect uncertainties (e.g., Luenberger observers \citep{conf:luenberger}), other approaches use stochastic to deal with uncertainties. Since observers considering stochastic processes are well-known (see e.g., \citep{conf:kfintro}), 
% Thus, many studies targeted the set-based state estimation, which becomes quite active in the past decades. 

%

%The most popular one is the statistical modeling of uncertainties. Kalman filter \citep{conf:kfintro} belongs to this category. Related work on this category puts statistical distribution assumption about the uncertainties. Assuming Gaussian distribution is the most widespread assumption on this category.  

%They make use of observer gain in an explicit way in order to take the effect of measurements in the state estimation operation . 

%Related work in \citep{conf:interval2asym} is constructed for time-invariant exponentially stable linear systems with additive disturbances and ensures that the error dynamics satisfy some conditions
%Authors in \citep{conf:interval4} used differential inequalities that allow deriving bounds for continuous differential systems at any time instant. 

\textbf{Interval-based observers:} These observers obtain possible sets of states by combining the model and the measurements through the observer gain \citep{conf:comparison} in order to bound state estimates by upper and lower bounds, which are obtained for instance from differential equations as in \citep{conf:interval1,conf:interval3}. By merging optimal and robust observer gain designs, a zonotopic Kalman Filter is proposed in \citep{conf:combastelzonotopes2}. Related work in \citep{conf:interval2asym} designs an exponentially stable interval observer for a two-dimensional time-invariant linear system. %The aforementioned work is extended for arbitrary finite dimension in \citep{conf:interval4}. The previous works on linear systems have been extended to nonlinear systems in \citep{conf:interval7,conf:interval8}. Another observer was proposed based on Muller’s theorem for nonlinear uncertain systems in \citep{conf:interval6bioreactor}. Also, authors in \citep{conf:h_inf} introduces $H_\infty$ design into interval estimation. Interval observers for uncertain biological systems are proposed in \citep{conf:interval5bio}.  %, or there may be 


% encloses the real state if the unknown initial state of the real system can be bounded. They generally provide specific information about the system trajectory at any instant given the bounds on the initial conditions, i.e., noise
%Interval observers are useful for dealing with uncertainty in fault detection applications. 

%We can more specifically classify the related work to a set-membership based approaches and interval observer-based approaches. 

%They also over-approximate the estimated states considering bounded uncertainties. 
\textbf{Set-membership-based observers:} They intersect the set of states consistent with the model and the set consistent with the measurements to obtain the corrected state set \citep{conf:intervalVSset-membership}. %In other words, they compute the set of admissible values for the state at each time instant.
One early example of set-membership-based observers is a recursive algorithm bounding the state by ellipsoids \citep{conf:1968}. Another early example based on normalized least-mean-squares (NLMS) is presented in \citep{conf:setmem4LMS}. A set-membership state estimation algorithm based on  %the difference of convex functions programming  
DC-programming is proposed in \citep{conf:setmem1dcprogramming}. Authors in \citep{conf:set_mem_discriptor} considers linear time-varying descriptor systems for set-membership estimation. %Set-memberships observers for nonlinear models are investigated in \citep{conf:setmem5,conf:setmem6,conf:setmem7,conf:setmem8,conf:set-mem-event}. They are also used in applications such as underwater robotics \citep{conf:setmem2water}, a leader following consensus problem in networked multi-agent systems \citep{conf:setmem3eventleader} and localization \citep{conf:setloc}. Authors in \citep{conf:disevent} consider a class of discrete time-varying system with an event-based communication mechanism over sensor networks. Interconnected multi-rate system is considered in \citep{conf:intermulti}. Set-membership with affine-projection is considered in \citep{conf:affineset}. Finally, nonlinear kernel adaptive filtering is proposed in \citep{conf:nonlinearset}.


%Different set representations of domains are used with set-membership based observers. For instance, ellipsoids are widely
%The symmetric properties of zonotopes help to reduce the computational load of using them iteratively. 

Different set representations have been used in set-based estimation, e.g, ellipsoids \citep{conf:set-ellipsoida},
orthotopes, and polytopes \citep{conf:orthotope,conf:polytope}. Zonotopes \citep{conf:zonotope_rep} are a special class of polytopes for which one can efficiently compute linear maps and Minkowski sums -- both are important operations for set-membership-based observers. A state bounding observer based on zonotopes is introduced in \citep{conf:zono1_Combastel}. Set-membership for discrete-time piecewise affine systems using zonotopes is studied in \citep{conf:zono2piecewise}. %Another work considers discrete-time descriptor systems in \citep{conf:zono_18pages}. Set-based estimation of uncertain discrete-time systems using zonotopes is proposed also in \citep{conf:zono4}.

%The zonotopic observer, in combination with Kalman filtering, is addressed in [6], [7]. 

%\textbf{Contributions:}
%In average consensus methods, the network must perform repeated averaging steps before arriving at a consensus. When these methods are used for distributed estimation, the nodes update their local estimates (using, for instance, a Kalman filter [6] or a leastsquares update [13]) and then they run a consensus step with several iterations to fuse the estimates. After the data have been fused, a new measurement is taken, the estimates are updated again, and so on. Thus, in consensus estimation algorithms there are two timescales: one for collecting the measurements, and one for running the averaging consensus.

%We consider the problem of distributed set-based estimation, where a set of nodes is required to collectively estimate the state set of a linear dynamic system from their measurements. 

\textbf{Contributions:} %Unlike centralized set-based estimation algorithms, which have potentially critical failure point at the central node, 
We propose distributed set-based estimators, where a set of nodes is required to collectively estimate the set of possible states of a linear dynamical system in a distributed fashion. 
%In traditional distributed set-based estimation, every node in a sensor-network receives the estimates based on its measurements only; then, the node intersects its set with the estimated sets of its neighbors  \citep{conf:dis-interconnected,conf:dis-kalmaninspired,conf:dis-partial}. However, we propose to let every node shares its measurements with its neighbor for faster convergence. 
We supplement our newly proposed observers with a set-based diffusion step, which intersects the shared state sets. Unlike prior efforts, we propose a new zonotopes intersection technique in the diffusion step, which reduces the over-approximation of the intersection results. We use the term \textit{diffusion} since our intersection formula resembles the traditional diffusion step in stochastic Kalman filter. In set-based estimation, the center of the set is considered as a single point estimate. We show that our diffusion step enhances the single point estimate and decreases the volume of the estimated sets. One main problem in distributed set-based estimation is the misalignment between the estimated sets by the distributed nodes, which would result in disagreements on fault detection results between nodes. This problem is usually solved by consensus methods \citep{conf:dis-consRR}. However, traditional consensus methods require the sensor network to perform several iterations before arriving at a consensus, which causes great overhead in set-based estimation. Our set-based diffusion step can be seen as lightweight approach to achieve partial consensus. One only obtains a partial consensus using our algorithms because every node has different neighbors with different measurements; thus, the resulting sets do not fully agree.% and we do not require running consensus iterations. 

More specifically, we make the following contributions:
\begin{itemize}
   % \item We propose two set-based algorithms, set-membership geometric shapes intersections inspires one algorithm, and the interval-based observer inspires the second one.
   \item We propose two distributed set-membership and interval-based algorithms combined with a new technique for intersection of zonotopes which is exploited in the proposed set-based diffusion step. 
 %   \item We propose a distributed set-membership algorithm, which is based on geometric intersections with.
 %   \item We propose a distributed interval-based algorithm, which is based on designing the observer gain.
 %   \item The diffusion step is proposed in both algorithms, where we introduce % can be done by alike convex combination between the shared sets.  
    \item We provide closed-forms for our parameter-finding optimization problems to realize faster execution times.
   % \item Our algorithms are evaluated using a localization example of a moving target. 
\end{itemize}
% Every node shares its measurement with its neighbor only in the measurement update step. Then, we find the intersection of the sets estimates between the neighbors to make the diffusion step in both algorithms. We propose our own zonotopes intersection in the diffusion step. Finally, the time update in the set-membership approach evolves the observer according to the system dynamics. The simplicity of matrix operations in dealing with zonotopes in comparison with polytopes motivates us to base our algorithms on zonotopes. %Our algorithms are useful in attack prevention \citep{conf:amrcdc2019} within a network of sensor nodes.

The rest of the paper is organized as follows: System model and preliminaries are in Section~\ref{sec:sysmodel}. In Section~\ref{sec:setmem}, we present the distributed set-membership diffusion observer as our first algorithm. Our second solution is the distributed interval-based diffusion observer which is introduced in Section~\ref{sec:berger}. Both algorithms are evaluated in Section~\ref{sec:eval}. Finally, we conclude the paper in Section~\ref{sec:conc}. 





